Interacting Hopf Algebras

We introduce the theory IH of interacting Hopf algebras, parametrised over a principal ideal domain R. The axioms of IH are derived using Lack's approach to composing PROPs: they feature two Hopf algebra and two Frobenius algebra structures on four different monoid-comonoid pairs. This construction is instrumental in showing that IH is isomorphic to the PROP of linear relations (i.e. subspaces) over the field of fractions of R.

==> source/3_Hermite.tex <==
Throughout the paper we fix a principal ideal domain (PID) $\PID = <R,0,1,+,\cdot>$. In this section we recall the basics of the theory of matrices with values in $\PID$, with particular attention to how their kernel (null space) can be computed. To this aim, we first recall a normal form for $\PID$-matrices called \emph{Hermite Normal Form}.

\begin{definition}\label{Def:HNF} An $m \times n$ matrix $A$ is said in Hermite Normal Form (HNF) if there is a natural number $r \leq n$ and a strictly increasing function $f \: [r+1,n] \to [1,m]$ associating column $i$ to a row $f(i)$, such that:
 \begin{enumerate}
   \item the first $r$ columns of $A$ have all entries with value $0$;
   \item for all columns $i$ with $r+1 \leq i \leq n$, $A_{f(i),i} \neq 0$ and
   \item for all $j \gr f(i)$, $A_{j,i} = 0$.
 \end{enumerate}
\end{definition}

There is an immediate observation stemming by the definition above.

\begin{lemma}\label{lemma:HNFtriangular} Suppose that $A$ is an $m \times n$ matrix in HNF and fix a column $i \leq n$. Then $A_{f(i),j} = 0$ for all columns $j \ls i$.
\end{lemma}
\begin{proof} If $j \leq r$ then $A_{f(i),j} = 0$ by property 1 of HNF. Otherwise, fix $j$ such that $r \ls j \ls i$. Since $f$ is strictly increasing, $f(i) \gr f(j)$. Then by property 3 of HNF, $A_{f(i),j} = 0$.
\qed\end{proof}

Hermite Normal Form generalizes Column Echelon Form to the setting of PIDs. Indeed, every $\PID$-matrix can be put into HNF by elementary column operations. We recall what those operations are:
\begin{description}
  \item[Column Swap] fixed $i,j \leq n$, replace column $C_i$ with $C_j$ and $C_j$ with $C_i$;
  \item[Column Sum] replace column $C_i$ with column $C_i + k C_j$, for some $k \in \PID$;
  \item[Unitary Multiplication] replace column $C_i$ with column $u C_i$, where $u \in \PID$ is a unitary element of the ring, i.e., it has a multiplicative inverse $u^{-1}$ in $\PID$.
\end{description}
For later reference, we also mention elementary row operations, which are defined by replacing ``column'' with ``row'' in each of the three items above.

\begin{proposition} Every $\PID$-matrix $A$ is column-equivalent to a unique matrix $B$ in HNF.
\end{proposition}
\begin{proof} See e.g. \cite{McDonald:linearalgebrarings,Cohen:1995ComputAlg} \qed\end{proof}

The transformation of $A$ into $B$ can be encoded as an invertible matrix $U$, obtained by applying to the identity matrix the sequence of elementary column operations allowing to pass from $A$ to $B$. Then $B = AU$ and we can compute from $U$ the kernel of $A$ as follows.

\begin{proposition}\label{prop:kernelfromHNF} For an $m \times n$ matrix $A$, let $B = AU$ be its HNF and $r \leq m$ the number of initial $0$-columns of $B$. Then the first $r$ columns of $U$ form a basis for the kernel of $A$.
\end{proposition}
\begin{proof} A proof can be found for the PID of integers in \cite[Prop. 2.4.9]{Cohen:1995ComputAlg}. We reformulate the same argument here for an arbitrary PID $\PID$.

For $i \leq r$, let $U_i$ be the $i$-th column of $U$. By definition $A U_i = B_i$, which is a $0$-vector because $i \leq r$. Thus all first $r$ columns of $U$ are elements of the kernel of $A$. Conversely, let $X$ be a vector such that $AX = 0$. Then $AX = A U U^{-1} X = B U^{-1} X$ because $U$ is invertible. Let $y_1, \dots, y_n$ be the entries of the vector $Y \df U^{-1}X$. For each $i$ in range $[r+1,n]$, we show that $y_i = 0$, by backward induction on $i$:
\begin{itemize}
  \item if $i =n$, let $f(n)$ be given as in Definition~\ref{Def:HNF}. Since $BY = 0$, then the $f(n)$-th entry of $BY$ is
      \begin{equation}\label{eq:propHNF1} \tag{$\bigtriangleup$}
          B_{f(n),1}y_1 + \dots + B_{f(n),n}y_n = 0.
      \end{equation}
      By Lemma~\ref{lemma:HNFtriangular}, $B_{f(n),1}, \dots, B_{f(n),{n-1}}$ are all equal to $0$, meaning by \eqref{eq:propHNF1} that $B_{f(n),n}y_n = 0$. By property 2 of HNF, $B_{f(n),n} \neq 0$ and thus, since $\PID$ has no non-zero divisors, $y_n = 0$.
  \item For $i$ with $r \ls i \ls n$, the $f(i)$-th entry of $BY$ is $B_{f(i),1}y_1 + \dots + B_{f(i),n}y_n = 0$ and by induction hypothesis $y_j = 0$ for all $j$ such that $i \ls j \leq n$. By Lemma~\ref{lemma:HNFtriangular}, $B_{f(i),1}, \dots, B_{f(i),{i-1}}$ are all equal to $0$, which means, analogously to the base case, that $B_{f(i),i}y_i = 0$ and since $B_{f(i),i}$ then $y_i = 0$.
\end{itemize}
Thus we proved that the entries $y_{r+1},\dots,y_n$ of $Y$ are equal to $0$. Instead the first $r$ entries of $Y$ can be arbitrary, because the $j$-th row of $BY$, for $j \leq r$, is give by $B_{j,1}y_1 + \dots + B_{j,n}y_n = 0$ and we know that, by property 1 of HNF, the entries $B_{j,1},\dots, B_{j,n}$ have value $0$.

Therefore the kernel of $B$ is generated by the first $r$ canonical basis vectors $C_1, \dots C_r$ of $\PID^n$. Since $B = AU$, then $UC_1, \dots, UC_r$ form a basis for the kernel of $A$. But those are just the first $r$ columns of $U$: hence we have proven the statement of the theorem.
\qed\end{proof}


